Near-Optimal Edge Evaluation in Explicit Generalized Binomial Graphs

Robotic motion-planning problems, such as a UAV flying fast in a partially-known environment or a robot arm moving around cluttered objects, require finding collision-free paths quickly. Typically, this is solved by constructing a graph, where vertices represent robot configurations and edges represent potentially valid movements of the robot between these configurations. The main computational bottlenecks are expensive edge evaluations to check for collisions. State of the art planning methods do not reason about the optimal sequence of edges to evaluate in order to find a collision free path quickly. In this paper, we do so by drawing a novel equivalence between motion planning and the Bayesian active learning paradigm of decision region determination (DRD). Unfortunately, a straight application of existing methods requires computation exponential in the number of edges in a graph. We present BISECT, an efficient and near-optimal algorithm to solve the DRD problem when edges are independent Bernoulli random variables. By leveraging this property, we are able to significantly reduce computational complexity from exponential to linear in the number of edges. We show that BISECT outperforms several state of the art algorithms on a spectrum of planning problems for mobile robots, manipulators, and real flight data collected from a full scale helicopter.

==> inputs/approach.tex <==
\section{The Bernoulli Subregion Edge Cutting Algorithm} \label{sec:algorithm}
We follow the framework of \emph{Decision Region Edge Cutting (\direct)}~\citep{chen2015submodular} by creating separate sub-problems for each region, and combining them. For each sub-problem, we provide a modification to \ecsq which is simpler to compute when the distribution over hypotheses is non-uniform, while providing the same guarantees. Unfortunately, naively applying this method requires $\bigo{2^\testSet}$ computation per sub-problem. For the special case of independent Bernoulli tests, we present a more efficient \emph{Bernoulli Subregion Edge Cutting (\algName)} algorithm, which computes each subproblem in $\bigo{\testSet}$ time. %Finally, we show how this computation can further be reduced to $\bigo{1}$ between iterations. 
We provide a brief exposition deferring to the supplementary for detailed derivations.

\subsection{A simple subproblem: One region versus all}
Following \citet{chen2015submodular}, we define a `one region versus all' subproblem, the solution of which helps address the \probBernDRD. Given a \emph{single region}, the objective is to either push the version space to that region, or collapse it to a single hypothesis. We view a region $\region$ as a version space $\regionH \subseteq \hypSpace$ consistent with its constituent tests. We define this subproblem over a set of \emph{disjoint subregions} $\subregion_i$. Let the hypotheses in the target region $\regionH$ be $\subregion_1$. Every other hypothesis $\hyp \in \Not{\regionH}$ is defined as its own subregion $\subregion_i, i>1$,  where $\Not{\regionH}$ is a set of hypothesis where a region is \emph{not} valid. Determining which subregion is valid falls under the framework of \emph{Equivalence Class Determination} (ECD), (a special case of the DRD problem) and can be solved efficiently by the \ecsq algorithm (\citet{golovin2010near}). This objective defines a graph with nodes as subregions and edges between distinct subregions, where the weight of an edge is the product of probabilities of subregions. As tests are performed and outcomes are received, the version space shrinks, decreasing the total weight of edges. Importantly, the problem is solved i.f.f. the weight of all edges is zero. The weight over the set of subregions is:
% The weight of all edges is:
% \sjnote{it's a little weird that later we use $\fec{argument}$ differently then $\ec$ here. One possibility: define a set of edges, define this as weights over them. You could even define this as a weight over the set of subregions, since that is what you define over.}
\begin{equation}
\label{eq:weight_golovin}
\wecgolovin(\{\subregion_i\}) %= \sum\limits_{i \neq j}  \weight(\subregion_i \times \subregion_j) 
= \sum\limits_{i \neq j} P(\subregion_i) P(\subregion_j)
\end{equation}
When hypotheses have uniform weight, this can be computed efficiently for the `one region versus all' subproblem. Let $P(\Not{\subregion_1}) =  \sum\limits_{i>1} P(\subregion_i)$:
\begin{equation}
    \wecgolovin(\{\subregion_i\}) = P(\subregion_1) P(\Not{\subregion_1}) + P(\Not{\subregion_1})\left(P(\Not{\subregion_1}) - \frac{1}{|\hypSpace|}\right)
\end{equation}
For non-uniform prior however, this quantity is more difficult to compute. We modify this objective slightly, adding self-edges on subregions $\subregion_{i}, i>1$, enabling more efficient computation while still maintaining the same guarantees:
\begin{equation}
\label{eq:weight_sub}
\begin{aligned}
    \wec(\{\subregion_i\}) &= P(\subregion_1) (\sum\limits_{i\neq1} P(\subregion_i)) + (\sum\limits_{i\neq1} P(\subregion_i)) (\sum\limits_{j \geq i} P(\subregion_j)) \\
    &= P(\subregion_1) P(\Not{\subregion_1}) + P(\Not{\subregion_1})^2 = P(\Not{\regionH}) (P(\regionH) + P(\Not{\regionH}))
\end{aligned}
\end{equation}
% \sjnote{Seems unecessary to define subregions? You compute all the quantities you need with $P(R)$ and $P(\Not R)$. Makes this more confusing}
For region $\region$, let the \emph{relevant version space} be $\hypSpaceR(\obsOutcome) = \setst{\hyp \in \hypSpace}{ \forall \test \in \selTestSet \cap \region, \hyp(\test) = \obsOutcome(\test)}$. The set of all hypotheses in $\regionH$ consistent with relevant outcomes in $\obsOutcome$ is given by $\regionH \cap \hypSpaceR(\obsOutcome)$. The terms $P(\regionH \cap \hypSpaceR(\obsOutcome))$ and $P(\Not{\regionH} \cap \hypSpaceR(\obsOutcome))$ allows us to quantify the progress made on determining region validity. Naively computing these terms would require computing all hypotheses and assigning them to correct subregions, thus requiring a runtime of $\bigo{2^\testSet}$. However, for the special case of Bernoulli tests, we can reduce this to $\bigo{\testSet}$ as we can see from the expression 
\begin{equation}
\wec(\{\subregion_i\} \cap \hypSpaceR(\obsOutcome) ) = \left(1 - \prod\limits_{i \in (\region \cap \selTestSet)} \Ind(\outcomeVarTest{i} = 1)
      \prod\limits_{j \in (\region \setminus \selTestSet)} \biasTest{j} \right)
      \left( \prod\limits_{k \in \region \cap \selTestSet} \biasTest{k}^{\obsOutcome(k)} (1 - \biasTest{k})^{1 - \obsOutcome(k)} \right)^2
\end{equation}
We can further reduce this to $\bigo{1}$ when iteratively updated (see supplementary for derivations).
We now define a criterion that incentivizes removing edges quickly and has theoretical guarantees. Let $\fec{\obsOutcome}$ be the weight of edges removed on observing outcome vector $\obsOutcome$. This is evaluated as
\begin{equation}
\begin{aligned}
\label{eq:fec_applied}
\fec{\obsOutcome} &= 1 - \frac{ \wec(\{\subregion_i\} \cap \hypSpaceR(\obsOutcome) ) }{ \wec(\{\subregion_i\}) }  \\
&= 1 - \frac{\left(1 - \prod\limits_{i \in (\region \cap \selTestSet)} \Ind(\outcomeVarTest{i} = 1)
      \prod\limits_{j \in (\region \setminus \selTestSet)} \biasTest{j} \right)
      \left( \prod\limits_{k \in \region \cap \selTestSet} \biasTest{k}^{\obsOutcome(k)} (1 - \biasTest{k})^{1 - \obsOutcome(k)} \right)^2
}{1 - \prod\limits_{i \in \region} \biasTest{i}}
\end{aligned}
\end{equation}

\begin{lemma}
The expression $\fec{\obsOutcome}$ is strongly adaptive monotone and adaptive submodular.
\end{lemma}

\subsection{Solving the \probBernDRD problem using \algName }

We now return to \probBernDRD problem (\ref{eq:drd}) where we have multiple regions $\{ \region_1, \dots, \region_\numRegion \}$ that overlap. Each region $\region_r$ is associated with an objective $\feci{r}{\obsOutcome}$ for solving the `one region versus all' problem. Since solving any one such subproblem suffices, we combine them in a \emph{Noisy-OR} formulation by defining an objective $\fdrd{\obsOutcome} = 1 - \prod\limits_{r=1}^\numRegion (1 - \feci{r}{\obsOutcome})$~\citep{chen2015submodular} which evaluates to
\begin{equation}
\label{eq:fdrd_applied}
\fdrd{\obsOutcome} =  1 - \prod\limits_{r=1}^\numRegion \left(  \frac{\left(1 - \prod\limits_{i \in (\region_r \cap \selTestSet)} \Ind(\outcomeVarTest{i} = 1)
      \prod\limits_{j \in (\region_r \setminus \selTestSet)} \biasTest{j} \right)
      \left( \prod\limits_{k \in \region_r \cap \selTestSet} \biasTest{k}^{\obsOutcome(k)} (1 - \biasTest{k})^{1 - \obsOutcome(k)} \right)^2
}{1 - \prod\limits_{i \in \region_r} \biasTest{i}}  \right)
\end{equation}
Since $\fdrd{\obsOutcome} = 1$ iff $\feci{r}{\obsOutcome} = 1$ for at least one $r$, we define the following surrogate problem to \probBernDRD 
\begin{equation}
\label{eq:direct_drd}
\policyOpt \in \argminprob{\policy} \;\cost(\policy) \; \mathrm{s.t} \; \forall \groundtruth \; : \;  \fdrd{\obsOutcomeFunc{\policy}{\groundtruth}} \geq 1
\end{equation}
The surrogate problem has a structure that allows greedy policies to have near-optimality guarantees
\begin{lemma}
The expression $\fdrd{\obsOutcome}$ is strongly adaptive monotone and adaptive submodular.
\end{lemma}

\begin{theorem}
\label{eq:drd_near_opt}
Let $\numRegion$ be the number of regions, $\pminH$ the minimum prior probability of any hypothesis, $\policy_{DRD}$ be the greedy policy and $\policyOpt$ with the optimal policy. Then $\cost(\policy_{DRD}) \leq \cost(\policy^*)(2\numRegion \log \frac{1}{\pminH} + 1)$.
\end{theorem}

\IncMargin{1em}
\begin{algorithm}[t]
  \caption{ Decision Region Determination with Independent Bernoulli Test$\left( \set{\region_i}_{i=1}^{\numRegion}, \biasVec, \groundtruth \right)$ }\label{alg:drd_skeleton}
  \algorithmStyle
  $\selTestSet \gets \emptyset$ \;
  \While{$(\nexists \region_i, P(\region_i | \obsOutcome) = 1) $ \textbf{\upshape and} $(\exists \region_i, P(\region_i | \obsOutcome) > 0) $}
  {
    $\candTestSet \gets \texttt{SelectCandTestSet}(\obsOutcome)$ \Comment*[r]{Using either (\ref{eq:cand_test_set:all}) or (\ref{eq:cand_test_set:maxp})}
    $\optTest \gets \texttt{SelectTest}(\candTestSet, \biasVec, \obsOutcome)$ \Comment*[r]{Using either (\ref{eq:greedy_fdrd}),(\ref{eq:policy_random}),(\ref{eq:policy_max_tally}),(\ref{eq:policy_set_cover}) or (\ref{eq:policy_mvoi})}  
    $\selTestSet \gets \selTestSet \cup \optTest$\; 
    $\outcomeTest{\optTest} \gets \groundtruth(\optTest)$ \Comment*[r]{Observe outcome for selected test}
  }
\end{algorithm}

We now describe the \algName algorithm. Algorithm \ref{alg:drd_skeleton} shows the framework for a general decision region determination algorithm. In order to specify \algName, we need to define two options - a candidate test set selection function $\texttt{SelectCandTestSet}(\obsOutcome)$ and a test selection function $\texttt{SelectTest}(\candTestSet, \biasVec, \obsOutcome)$. The unconstrained version of \algName implements $\texttt{SelectCandTestSet}(\obsOutcome)$ to return the set of all tests $\candTestSet$ that contains only unevaluated tests belonging to active regions
\begin{equation}
  \label{eq:cand_test_set:all}
  \candTestSet = \set{\bigcup\limits_{i=1}^\numRegion \setst{\region_i}{P(\region_i | \obsOutcome) > 0}}
  \setminus \selTestSet
\end{equation}
We now examine the \algName test selection rule $\texttt{SelectTest}(\candTestSet, \biasVec, \obsOutcome)$   
\begin{equation}
\begin{aligned}
\label{eq:greedy_fdrd}
\test^*  &\in  \argmaxprob{\test \in \candTestSet}\; \frac{1}{\cost(\test)} \mathbb{E}_{\outcomeTest{\test}} \left[ 
       \prod\limits_{r=1}^\numRegion  
      \left(1 - \prod\limits_{i \in (\region_r \cap \selTestSet)} \Ind(\outcomeVarTest{i} = 1) \prod\limits_{j \in (\region_r \setminus \selTestSet)} \biasTest{j} \right) \right.\\
      & - \left. \left( \prod\limits_{r=1}^\numRegion 
      \left(1 - \prod\limits_{i \in (\region_r \cap \selTestSet \cup \test)} \Ind(\outcomeVarTest{i} = 1) \prod\limits_{j \in (\region_r \setminus \selTestSet \cup \test)} \biasTest{j} \right) \right)
      ( \biasTest{t}^{\outcomeTest{\test}} (1-\biasTest{t})^{1-\outcomeTest{\test}} )^{2\sum\limits_{k=1}^{m} \Ind(\test \in \region_k)} \right]
\end{aligned}
\end{equation}
The intuition behind this update is that tests are selected to squash the probability of regions not being valid. It also additionally incentivizes selection of tests on which multiple regions overlap. 
\subsection{Adaptively constraining test selection to most likely region}
We observe in our experiments that the surrogate (\ref{eq:fdrd_applied}) suffers from a slow convergence problem - $\fdrd{\obsOutcome}$ takes a long time to converge to $1$ when greedily optimized. 
%This can be attributed to the curvature of the function (Fig.~\ref{fig:histogram_max_prob}).  
To alleviate the convergence problem, we introduce an alternate candidate selection function $\texttt{SelectCandTestSet}(\obsOutcome)$ that assigns to $\candTestSet$ the set of all tests that belong to the most likely region $\maxProbTestSet$ which is evaluated as follows (we will refer to this variant as \algMaxProbReg)
\begin{equation}
  \label{eq:cand_test_set:maxp}
  \maxProbTestSet = \set{\argmaxprob{\region_i = \seq{\region}{\numRegion}}  \;P(\region_i | \obsOutcome) }
  \setminus \selTestSet
\end{equation}
Applying the constraint in (\ref{eq:cand_test_set:maxp}) leads to a dramatic improvement for any test selection policy as we will show in Sec.~\ref{sec:experiments:discussion}. The following theorem offers a partial explanation
\begin{theorem}
A policy that greedily latches to a region according the the posterior conditioned on the region outcomes has a near-optimality guarantee of 4 w.r.t the optimal region evaluation sequence.
\end{theorem}
Applying the constraint in (\ref{eq:cand_test_set:maxp}) implies we are no longer greedily optimizing $\fdrd{\obsOutcome}$. However, the following theorem bounds the sub-optimality of this policy. 
\begin{theorem}
  Let $\pmin = \min_i P(\region_i)$, $\pminH = \min_{\hyp \in \hypSpace} P(\hyp)$ and $l = \max_i \abs{\region_i}$. The policy using (\ref{eq:cand_test_set:maxp}) has a suboptimality of $\alpha \left(2 \numRegion \log \left( \frac{1}{\pminH} \right) + 1 \right)$ where 
$\alpha \leq \left( 1 -   \max \left( (1 - \pmin)^2, \pmin^{\frac{2}{l}} \right) \right)^{-1}$.
\end{theorem} \vspace{-0.5em}


==> inputs/experiments.tex <==
\section{Experiments} \vspace{-0.7em}
\label{sec:experiments}
We evaluate \algName on a collection of datasets spanning across a spectrum of synthetic problems and real-world planning applications. 
The synthetic problems are created by randomly selecting problem parameters to test the general applicability of \algName.
The motion planning datasets range from simplistic yet insightful 2D problems to more realistic high dimension problems as encountered by an UAV or a robot arm. 
The 7D arm planning dataset is obtained from a high fidelity simulation as shown in Fig.~\ref{fig:real_world_planning}(a).
Finally, we test \algName on experimental data collected from a full scale helicopter flying that has to avoid unmapped wires at high speed as it comes into land as shown in Fig.~\ref{fig:real_world_planning}(b).
Refer to supplementary for exhaustive details on experiments and additional results. \footnote{We plan to provide a link to open source code and datasets for the camera ready version.}
%\sjnote{Seems like some datasets are missing? I would also sell this a little harder, especially for the real problems}

\subsection{Heuristic approaches to solving the \probBernDRD problem} \vspace{-0.7em}
\label{sec:heuristics}
%\sjnote{Move this to experiments section, make it a subsection?}
We propose a collection of competitive heuristics that can also be used to solve the \probBernDRD problem. These heuristics are various $\texttt{SelectTest}(\candTestSet, \biasVec, \obsOutcome)$ policies in the framework of Alg.~\ref{alg:drd_skeleton}. To simplify the setting, we assume unit cost $\cost(\test) = 1$ although it would be possible to extend these to nonuniform setting. The first heuristic \algRandom selects a test by sampling uniform randomly
\begin{equation}
  \label{eq:policy_random}
  \optTest \in \candTestSet
\end{equation}
We adopt our next heuristic \algMaxTally from \citet{dellin2016unifying} where the test belonging to most regions is selected. It uses the following criteria, which exhibits a `fail-fast' characteristic
\begin{equation}
  \label{eq:policy_max_tally}
  \optTest   \in  \argmaxprob{\test \in \candTestSet}\; \sum\limits_{i=1}^{\numRegion} \Ind\left(\test \in \region_i, P(\region_i | \obsOutcome) > 0 \right)
\end{equation}
The next policy \algSetCover selects tests that maximize the expected number of `covered' tests, i.e. if a selected test is in collision, how many other tests does it remove from consideration.
\begin{equation}
  \label{eq:policy_set_cover}
  \optTest \in  \argmaxprob{\test \in \candTestSet}\; 
  (1 - \biasTest{\test})
  \abs{ 
  \set{\bigcup\limits_{i=1}^\numRegion \setst{\region_i}{P(\region_i | \obsOutcome) > 0} - 
  \bigcup\limits_{j=1}^\numRegion \setst{\region_j}{P(\region_j | , \substack{\obsOutcome, \\ \outcomeVarTest{\test} = 0} ) > 0}   }
  \setminus \set{\selTestSet \cup \set{\test}}
  } 
\end{equation}
\begin{theorem}
\algSetCover is a near-optimal policy for the problem of optimally checking all regions. 
\end{theorem}
The last baseline is derived from a classic heuristic in decision theory: myopic value of information (\citet{howard1966information}). 
\algMVOI greedily chooses the test that maximizes the change in the probability mass of the most likely region. This test selection works only with $\texttt{SelectCandTestSet}(\obsOutcome) = \maxProbTestSet$. 
\begin{equation}
  \label{eq:policy_mvoi}
  \optTest   \in  \argmaxprob{\test \in \maxProbTestSet}\; (1 - \biasTest{\test}) \max\limits_{i = 1, \dots, \numRegion} P(\region_i \;|\; \obsOutcome, \outcomeVarTest{\test} = 0)
\end{equation}



\begin{figure}[t]
    \centering
    \includegraphics[page=1,width=\textwidth]{2d_env_comparison.pdf}
    \caption{%
    \label{fig:2d_env_comparison}
    Performance (number of evaluated edges) of all algorithms on 2D geometric planning. Snapshots, at interim and final stages respectively, show evaluated valid edges (green), invalid edges (red) and the final path (magenta). The utility of edges as computed by algorithms is shown varying from low (black) to high (cream).}
\end{figure}%

\begin{figure}[t]
    \centering
    \includegraphics[page=1,width=\textwidth]{real_world_planning.pdf}
    \caption{%
    \label{fig:real_world_planning}
    (a) A 7D arm has to perform pick and place tasks at high speed in a table with clutter. (b) Experimental data from a full-scale helicopter that has to react quickly to avoid unmapped wires detected by the sensor. \algName (given an informative prior) checks a small number of edges around the detected wire and identifies a path. (c) Scenario where regions have size disparity. Unconstrained \algName significantly outperforms other algorithms on such a scenario.
    \fullFigGap}
\end{figure}%

\input{figs/table2}
\vspace{-0.7em}
\subsection{Analysis of results} \vspace{-0.7em}
\label{sec:experiments:discussion}
Table~\ref{tab:benchmark_results} shows the evaluation cost of all algorithms on various datasets normalized w.r.t \algName. The two numbers are lower and upper $95\%$ confidence intervals - hence it conveys how much fractionally poorer are algorithms w.r.t \algName. The best performance on each dataset is highlighted. We present a set of observations to interpret these results.
\begin{observation}
\algName has a consistently competitive performance across all datasets.
\end{observation} \vspace{-0.7em}

Table~\ref{tab:benchmark_results} shows on $13$ datasets, \algName is at par with the best - on $8$ of those it is exclusively the best. 

\begin{observation}
The \algMaxProbReg variant improves the performance of all algorithms on most datasets
\end{observation} \vspace{-0.7em}

Table~\ref{tab:benchmark_results} shows that this is true on $12$ datasets. The impact is greatest on \algRandom where improvement is upto a factor of $20$. However, this is not true in general. On datasets with large disparity in region sizes as illustrated in Fig.~\ref{fig:real_world_planning}(c), unconstrained \algName significantly outperforms other algorithms. In such scenarios, \algMaxProbReg latches on to the most probable path which also happens to have a large number of edges. It performs poorly on instances where this region is invalid, while the other region containing a single edge is valid. Unconstrained \algName prefers to evaluate the single edge belonging to region 1 before proceeding to evaluate region 2, performing optimally on those instances. Hence, the myopic nature of \algMaxProbReg is the reason behind its poor performance.
\begin{observation}
On planning problems, \algName strikes a trade-off between the complimentary natures of \algMaxTally and \algMVOI.
\end{observation} \vspace{-0.7em}

We examine this in the context of 2D planning as shown in Fig.~\ref{fig:2d_env_comparison}. 
\algMaxTally selects edges belonging to many paths which is useful for path elimination but does not reason about the event when the edge is not in collision.
\algMVOI selects edges to eliminate the most probable path but does not reason about how many paths a single edge can eliminate. 
\algName switches between these behaviors thus achieving greater efficiency than both heuristics.

\begin{observation}
\algName checks informative edges in collision avoidance problems encountered a helicopter
\end{observation} \vspace{-0.7em}

Fig.~\ref{fig:real_world_planning}(b) shows the efficacy of \algName on experimental flight data from a helicopter avoiding wire.
